On Leveraging Variational Graph Embeddings for Open World Compositional Zero-Shot Learning

Humans are able to identify and categorize novel compositions of known concepts. The task in Compositional Zero-Shot learning (CZSL) is to learn composition of primitive concepts, i.e. objects and states, in such a way that even their novel compositions can be zero-shot classified. In this work, we do not assume any prior knowledge on the feasibility of novel compositions i.e.open-world setting, where infeasible compositions dominate the search space. We propose a Compositional Variational Graph Autoencoder (CVGAE) approach for learning the variational embeddings of the primitive concepts (nodes) as well as feasibility of their compositions (via edges). Such modelling makes CVGAE scalable to real-world application scenarios. This is in contrast to SOTA method, CGE, which is computationally very expensive. e.g.for benchmark C-GQA dataset, CGE requires 3.94 x 10^5 nodes, whereas CVGAE requires only 1323 nodes. We learn a mapping of the graph and image embeddings onto a common embedding space. CVGAE adopts a deep metric learning approach and learns a similarity metric in this space via bi-directional contrastive loss between projected graph and image embeddings. We validate the effectiveness of our approach on three benchmark datasets.We also demonstrate via an image retrieval task that the representations learnt by CVGAE are better suited for compositional generalization.

==> MIT-States.tex <==
\begin{table}
\centering
\begin{tabular}{|l|ccc|}
\hline
Method & R@1 & R@5 & R@10\\
\hline\hline
% Image only & 3.3$^{\pm0.1}$ & 12.8$^{\pm0.2}$ & 20.9$^{\pm0.1}$\\
% Text only & 7.4$^{\pm0.4}$ & 21.5$^{\pm0.9}$ & 32.7$^{\pm0.8}$\\
%\hline
% PM -- projection module
% Concatenation & 11.8$^{\pm0.2}$ & 30.8$^{\pm0.2}$ & 42.1$^{\pm0.3}$ \\
Show and Tell & 11.9$^{\pm0.1}$ & 31.0$^{\pm0.5}$ & 42.0$^{\pm0.8}$ \\
Att. as Operator  & 8.8$^{\pm0.1}$ & 27.3$^{\pm0.3}$ & 39.1$^{\pm0.3}$ \\
Relationship  & 12.3$^{\pm0.5}$ & 31.9$^{\pm0.7}$ & 42.9$^{\pm0.9}$ \\
FiLM  & 10.1$^{\pm0.3}$ & 27.7$^{\pm0.7}$ & 38.3$^{\pm0.7}$ \\
TIRG & 12.2$^{\pm0.4}$ & 31.9$^{\pm0.3}$ & 43.1$^{\pm0.3}$\\
\hline

TIRG with BERT & {12.3}$^{\pm0.6}$ & {31.8}$^{\pm0.3}$ & {42.6}$^{\pm0.8}$  \\
TIRG with &  &  & \\ Complete Text Query & 7.9$^{\pm 1.9}$ & 28.7$^{\pm 2.5}$ & 34.1$^{\pm2.9}$  \\
% TIRG with &  &  & \\ Complete Text Query & 12.9$^{\pm 0}$ & 33.7$^{\pm 0}$ & 44.1$^{\pm0}$  \\
% runs TIRG with complete text query 54k iterations
% r1: 0.03714, 0.05374
% r5: 0.11, 0.1752
% r10: 0.1781, 0.2511
\hline

TIRG with BERT and &&&\\ Complete Text Query & \underline{13.3}$^{\pm0.6}$ & \underline{34.5}$^{\pm1.0}$ & \underline{46.8}$^{\pm1.1}$ \\
% & 13.6$^{\pm0.9}$  & 35.5$^{\pm0.8}$  & 47.4$^{\pm1.1}$  \\
% saturated 66k: & {13.3}$^{\pm0.6}$ & {34.5}$^{\pm1.0}$ & {46.8}$^{\pm1.1}$ 
\hline
ComposeAE & \textbf{13.9}$^{\pm0.5}$ & \textbf{35.3}$^{\pm0.8}$ & \textbf{47.9}$^{\pm0.7}$\\ %https://workflowy.com/#/e9f3c5bb2d4a % ...

\hline
\end{tabular}
% \vspace{3mm}
\caption{Model performance comparison on MIT-States. The best number is in bold and the second best is underlined.}
\label{tab:mitstates}
\end{table}


==> ablation_arch_loss.tex <==

\begin{table}[ht]
\centering
\scalebox{0.85}{
\begin{tabular}{|l|ccc|}
\hline
Method     & Fashion200k & MIT-States & Fashion IQ \\
\hline\hline
ComposeAE  &   55.3    &       47.9    & 11.8    \\
 \hline
  - without $L_{SYM}$  &  51.6     &  47.6    & 10.5 \\
 - Concat in real space   &   48.4      & 46.2   & 09.8  \\ 
 \hline
 - without $\rho_{conv}$  &  52.8      &  47.1    & 10.7  \\
 - without $\rho$     &  52.2    &  45.2   &  11.1 \\
 \hline
% L2 Dec losses play a significant role in stabilizing the learning process. Variation is huge, without them.
% https://workflowy.com/#/843f6123b7fb

\end{tabular}}
\vspace{2mm}
\caption{\label{tab:ablation}Retrieval performance (R@10) of ablation studies.}
\end{table}

==> f200k.tex <==

\begin{table}[ht]

\centering

% \resizebox{0.9}
{\begin{tabular}{|l|ccc|}
\hline
Method & R@1 & R@10 & R@50 \\
\hline\hline
Han \etal~\cite{han2017automatic}  & 6.3 & 19.9 & 38.3 \\
% Image only & 3.5 & 22.7 & 43.7 \\
% Text only & 1.0 & 12.3 & 21.8 \\
%\hline
% Concatenation & 11.9$^{\pm1.0}$ & 39.7$^{\pm1.0}$ & \underline{62.6}$^{\pm0.7}$ \\
Show and Tell & 12.3$^{\pm1.1}$ & 40.2$^{\pm1.7}$ & 61.8$^{\pm0.9}$ \\
Param Hashing & 12.2$^{\pm1.1}$ & 40.0$^{\pm1.1}$ & 61.7$^{\pm0.8}$ \\
Relationship & {13.0}$^{\pm0.6}$ & {40.5}$^{\pm0.7}$ & 62.4$^{\pm0.6}$ \\
FiLM  & 12.9$^{\pm0.7}$ & 39.5$^{\pm2.1}$ & 61.9$^{\pm1.9}$ \\
TIRG & {14.1}$^{\pm0.6}$ & {42.5}$^{\pm0.7}$ & {63.8}$^{\pm0.8}$ \\
\hline
TIRG with BERT & 14.2$^{\pm1.0}$ & 41.9$^{\pm1.0}$ & 63.3$^{\pm0.9}$  \\
TIRG with &  &  & \\ Complete Text Query & 18.1$^{\pm1.9}$ & \underline{52.4}$^{\pm2.7}$ & \underline{72.1}$^{\pm2.1}$  \\
% TIRG with &  &  & \\ Complete Text Query & 18.1$^{\pm0}$ & 47.4$^{\pm0}$ & 69.8$^{\pm0}$  \\
% runs TIRG with complete text query 59k iterations
% r1: 0.1779, 0.1547, 0.1797
% r10: 0.5546, 0.482, 0.512
% r50: 0.7418, 0.7767, 0.7535

\hline
TIRG with BERT and &  &  & \\ Complete Text Query & \underline{19.9}$^{\pm1.0}$ & {51.7}$^{\pm1.5}$ & {71.8}$^{\pm1.3}$  \\
\hline
ComposeAE & \textbf{22.8}$^{\pm0.8}$ & \textbf{55.3}$^{\pm0.6}$ & \textbf{73.4}$^{\pm0.4}$ \\
\hline
\end{tabular}}

\label{tab:f200k}
% \vspace{3mm}
\caption{Model performance comparison on Fashion200k. The best number is in bold and the second best is underlined.}
\end{table}


==> fiq.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.89\linewidth]{FIQ_Retrieval.jpg}
\caption{Qualitative Results: Retrieval examples from FashionIQ Dataset}
\label{fig:fIQqual}
\end{figure*}


\begin{table}[ht]

\centering
\begin{tabular}{|l|ccc|}
\hline
Method & R@10 & R@50 & R@100 \\
\hline\hline
TIRG with &  &  & \\ Complete Text Query & 3.34$^{\pm0.6}$  & 9.18$^{\pm0.9}$  &  9.45$^{\pm0.8}$ \\
% saturated 17k: & {3.4}$^{\pm0.7}$ & {9.1}$^{\pm0.6}$ & {9.11}$^{\pm0.6}$ 
\hline
TIRG with BERT and &  &  & \\ Complete Text Query & \underline{11.5}$^{\pm0.8}$ & \underline{28.8}$^{\pm1.5}$ & \underline{28.8}$^{\pm1.6}$
% saturated 17k: & {11.5}$^{\pm0.7}$ & {28.8}$^{\pm1.5}$ & {28.8}$^{\pm1.6}$ 
\\
\hline
ComposeAE & \textbf{11.8}$^{\pm0.9}$ & \textbf{29.4}$^{\pm1.1}$ & \textbf{29.9}$^{\pm1.3}$ \\

\hline
\end{tabular}

\label{tab:fiq}
\vspace{3mm}
\caption{Model performance comparison on Fashion IQ. The best number is in bold and the second best is underlined.}
\end{table}


% The main difference between experiments on Fashion-IQ and two other datasets is that in former the algorithm is supposed to rank and retrieve images which haven't seen by the algorithm in the training pipeline just by using the text query. In two other datasets, in the way they have been constructed lies an implicit bias: a small vocabulary and short number of transitions between each of the objects. That's why in the wildest of conditions when both the image domain is the same for all images and text description is fairly complex (case for fashion200k and fashionIQ, not MITStates) and the inference runs on the unknown images which haven't been in train, TIRG appoarch fails to place similar images together in high-dimensional ranking space. Firstly, because of the failing in providing a complex context embedding with TIRG original LSTM and secondly, not able to correctly place the images in the space having the complex context embedding provided by BERT (because of not treating the text feature properly).

% Sidenotes:

% I guess we should focus on the idea that it is necessary to provide a rich text embedding in order to learn a rich multi-modal representation and the learned multi-modal representation should possess the properties we constraint it within the solution space as you wrote above in the paper.
